A baseline for unsupervised advanced persistent threat detection in system-level provenance

Advanced persistent threats (APT) are stealthy, sophisticated, and unpredictable cyberattacks that can steal intellectual property, damage critical infrastructure, or cause millions of dollars in damage. Detecting APTs by monitoring system-level activity is difficult because manually inspecting the high volume of normal system activity is overwhelming for security analysts. We evaluate the effectiveness of unsupervised batch and streaming anomaly detection algorithms over multiple gigabytes of provenance traces recorded on four different operating systems to determine whether they can detect realistic APT-like attacks reliably and efficiently. This report is the first detailed study of the effectiveness of generic unsupervised anomaly detection techniques in this setting.

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

The ingester and user interface discussed in
Section~\ref{sec:overview} are implemented in Scala.  Provenance
records representing system activity are read from a Kafka topic or
file.  The system maintains some history regarding previously-ingested
data in order to facilitate duplicate elimination or extraction of
contexts.  The ingested data is also stored in a Neo4j database, and
contexts can also be extracted from that after the fact.  The contexts
used for the experiments were extracted in this way, using simple
queries and Python scripts.  It is straightforward to extract the
contexts from the data as it is ingested, by maintaining records
summarizing each process's behavior and output each record when the
associated process terminates.  For long-running processes, we can
generate one record summarizing the behavior over an extended period
(for example, a day or the entire run).

We have implemented the anomaly detection approaches described in
Section~\ref{sec:methods} in Python.  Each approach works in a similar
way.  For the batch algorithm, we first scan the data to count the
number of attribute value occurrences, and then rescan to score each
record as described in Section~\ref{sec:methods}.  For the online
algorithm, a single scan is performed in each case.  The online
algorithm can also process fixed-size blocks of records instead of
just one record at a time.  The total code size is under 500 lines of
code, including a naive but readable implementation used for initial
exploration and an optimized version used for the experimental
results.

